Wiretap Secret Key Agreement Via Secure Omniscience

In this paper, we explore the connection between secret key agreement and secure omniscience within the setting of the multiterminal source model with a wiretapper who has side information. While the secret key agreement problem considers the generation of a maximum-rate secret key through public discussion, the secure omniscience problem is concerned with communication protocols for omniscience that minimize the rate of information leakage to the wiretapper. The starting point of our work is a lower bound on the minimum leakage rate for omniscience, $R_{\mathop{\mathrm{L}}}$, in terms of the wiretap secret key capacity, $C_{\mathop{\mathrm{W}}}$. Our interest is in identifying broad classes of sources for which this lower bound is met with equality, in which case we say that there is a duality between secure omniscience and secret key agreement. We show that this duality holds in the case of certain finite linear source (FLS) models, such as two-terminal FLS models and pairwise independent network models on trees with a linear wiretapper. Duality also holds for any FLS model in which $C_{\mathop{\mathrm{W}}}$ is achieved by a perfect linear secret key agreement scheme. We conjecture that the duality in fact holds unconditionally for any FLS model. On the negative side, we give an example of a (non-FLS) source model for which duality does not hold if we limit ourselves to communication-for-omniscience protocols with at most two (interactive) communications. We also address the secure function computation problem and explore the connection between the minimum leakage rate for computing a function and the wiretap secret key capacity.

==> conclusion.tex <==
For a tree-PIN model with linear wiretapper, we have characterized $\rl$ and $\wskc$. It is worth noting that since the evaluation of the lower bound on $\wskc$ given in \cite[Th. 7]{aminsource} is not explicit, the optimality of the bound is not very clear. But we showed an even stronger result for our particular model that a linear secure omniscience scheme achieves $\wskc$, which establishes the duality between the two problems. So, our result gives evidence for the conjecture that, for FLSs, secure omniscience achieves $\wskc$. However, proving this even for a general PIN model turned out to be quite challenging. Another interesting part of the proof is the communication scheme that achieves perfect omniscience and perfect alignment with the wiretapper. Though we used a random coding approach in the proof, there is an explicit optimal protocol construction in the case $n_e=1$ for all $e \in E$ \cite[Sec. V]{treepin21arxiv}. Such deterministic protocols, which have potential application in the CCDE context, are not known in the general tree-PIN case. 


==> explicitprotocol.tex <==
In the proof of Theorem \ref{thm:cwsk:irred}, we have fixed the communication matrix structure and argued, using the probabilistic method, that if $n > \log_q sL$ then there exist communication coefficients  that achieve $\rl$. To that end, we first showed the existence of a realization of an $\MS$ such that $\MS\MW^{(n)}=0$ and $\MS_i$'s are invertible. Since $\MS$ and communication coefficients are recoverable from each other, the desired existence follows. However, in the case when $n_e=1$ for all $e \in E$, we give an explicit way to find these coefficients and the sufficient $n$ to do this. Here $\MS$ is just a row vector with entries from $\bb{F}_{q^n}$. Our goal is to find a vector with non-zero entries from $\bb{F}_{q^n}$  for some $n$ such that it satisfies $\MS\MW^{(n)} =\M0$.  Note that $\MW^{(n)}$ is a $\left(\sum_{e \in E} n_e\right) \times n_w$ matrix over $\bb{F}_{q^n}$ with entries $\MW^{(n)}(k,l) = \MW(k,l) \in  \bb{F}_{q}$; since $\bb{F}_{q} \subseteq \bb{F}_{q^n}$, $\MW^{(n)}(k,l) \in \bb{F}_{q^n}$. In the proof of the  following lemma, we actually show how to choose $\MS$.
 \begin{lemma}
  Let $\MW$ be an $(m+k) \times m$ matrix over $\Fq$ and $k,m \geq 1$. Assume that the columns of $\MW$ are linearly independent. If the span of the columns of $\MW$ does not contain any vector that is a scalar multiple of any standard basis vector, then there exists an $1 \times  (m+k)$ vector $\MS$ whose entries belong to $\mathbb{F}_{q^k}^{\times} := \mathbb{F}_{q^k} \backslash \{0\}$ such that $\MS\MW^{(k)}=0$.
 \end{lemma}
 \begin{proof}
  Since the columns of $\MW$ are linearly independent, we can apply elementary column operations and row swappings on the matrix $\MW$ to reduce into the form $\tMW=[\MI_{m\times m} \mid \MA_{m \times k}]^T$, for some matrix $\MA_{m \times k}$. It means that $\tMW=\MP\MW\MC$ for some permutation matrix $\MP$ and an invetible matrix $\MC$ corresponding to the column operations. Furthermore, the matrix $\MA_{m \times k}$ has no zero rows because if there were a zero row in $\MA$ then the corresponding column of $\tMW$ is a standard basis vector which means that the columns of $\MW$ span a standard basis vector contradicting the hypothesis.
  
  Now consider the field $\mathbb{F}_{q^k}$. The condition $\MS\MW^{(k)} =0$ can be written as  $\tMS\tMW^{(k)} = 0$ where $\tMW^{(k)}=\MP\MW^{(k)}\MC$ and $\tMS=\MS\MP^{-1}$. Since $\mathbb{F}_{q^k}$ is a vector space over $\Fq$, there exists a basis  $\{\beta_1, \beta_2, \ldots, \beta_k\} \subset \mathbb{F}_{q^k}$. We will use this basis to construct $\tMS$ and hence $\MS$. For $\MA=[a_{ij}]_{i \in [m], j \in [k]}$, set $\tMS_{m+i} = \beta_i\neq 0$ for $i \in [k]$ and $\tMS_i = - \sum_{j=1} ^{k} a_{ij}\beta_j \neq 0$ for $i \in [m]$. So all entries of $\tMS$  are non-zero entries which follows from the fact that $\beta_j$'s are linearly independent and for a fixed $i$, $a_{ij}$'s are not all zero. Therefore we found an $\tMS$ such that $\tMS\tMW^{(k)} = \M0$. This in turns gives $\MS$, which is obtained by permuting the columns of $\tMS$, such that $\MS\MW^{(k)} = \M0$.
 \end{proof}
 
 In the case when $n_e=1$ and the source is irreducible, the wiretapper matrix satisfies the conditions in the hypothesis of the above lemma. Therefore, we can use the construction given in that lemma to find an $\MS$  such that $\MS\MW^{(n)}=0$ where $n = |E|-n_w$. From $\MS$, we can recover back the communication coefficients $\MA_{i,e} \in \mathbb{F}_{q^k}$ because  given all $\MS_e$ along the unique path from $i$ to the root node, we can recursively compute all $\MA_{i,e}$ along that path. 
 
 We could not extend these ideas beyond this case but it is worth finding such simple and explicit constructions in the arbitrary $n_e$ case. Another interesting question is, for a given tree-PIN source with linear wiretapper, what is the minimum $n$ required to achieve perfect omniscience and perfect alignment using a linear communication? Note that the $n$ required in our protocol is $|E|-n_w$ whereas the  probabilistic method guarantees a scheme if $n > \log_q|E|$. So we clearly see that  $n = |E|-n_w$  is not optimal in some cases. 
 

==> positivity.tex <==
In this section, we will use the inequality $H(\RZ_V|\RZ_{\opw}) - \wskc \leq \rl$ to establish an equivalent condition for the positivity of $\wskc$. This result extends the two-user result of \cite[Theorem~4]{amin2020} to the multiuser case. In the two-user setting \cite{amin2020}, Gohari, G\"{u}nl\"{u} and Kramer studied the positivity of $\wskc$, and gave an equivalent characterization in terms of R\'enyi divergence by using hypothesis testing and a coding scheme that involves repetition with block-swapping. This coding idea remains one of the main ingredients of our proof.

For two distributions $P_{\RX}$ and $P_{\tRX}$ on a common alphabet $\mc{X}$, the \emph{R\'enyi divergence of order $1/2$} between $P_{\RX}$ and $P_{\tRX}$ is given by $D_{\frac{1}{2}}(P_{\RX} \| P_{\tRX}):=-2\log\left( \sum_{x \in \mc{X}} \sqrt{P_{\RX}(x)P_{\tRX}(x)}\right),$
and the total variation (TV) distance between  $P_{\RX}$ and $P_{\tRX}$ is given by ${\|P_{\RX}-P_{\tRX}\|}_{\mathrm{TV}}:=\frac{1}{2}\sum_{x \in \mc{X}}|P_{\RX}(x)-P_{\tRX}(x)|$.
To state the theorem, let us define $\Delta(\RZ_V \| \RZ_{\opw}) := \inf {\|P_{\RK_1,\ldots, \RK_m,\RF^{(n)},\RZ^n_{\opw}}-\dfrac{1}{2}\mathbf{1}_{\RK_1=\dots=\RK_m}\cdot P_{\RF^{(n)},\RZ^n_{\opw}}\|}_{\mathrm{TV}}$ where the infimum is over all communication schemes and possible binary keys (see \cite[Def.~8]{amin2020}). 

\begin{theorem}\label{thm:multivariate_positivity}
 For a source $(\RZ_1,\ldots,\RZ_m,\RZ_{\opw})$ with distribution $P_{\RZ_1 \ldots \RZ_m \RZ_{\opw}}$ and $m \geq 2$, the following statements are equivalent:
 \begin{enumerate}
  \item There is an integer $r$ and non-empty disjoint sets $\mc{A}_{11},\mc{A}_{12} \subset \mc{Z}_1^r$, $\mc{A}_{21},\mc{A}_{22} \subset \mc{Z}_2^r$, $\ldots, \mc{A}_{m1},\mc{A}_{m2} \subset \mc{Z}_m^r$ such that
  \begin{align*}
       &D_{\frac{1}{2}} \left(P_{\RZ_{\opw}^r}(\cdot \mid \mc{E}_{1, 1, \ldots, 1})  
       %\right. \\& \mkern 100mu \left.
       \| P_{\RZ_{\opw}^r}(\cdot \mid \mc{E}_{2, 2, \ldots, 2}) \right)%\\ & 
       < \log \left(\frac{\Pr(\mc{E}_{1, \ldots, 1})\Pr(\mc{E}_{2, \ldots, 2})}{\sum \limits_{\substack{(j_1,\ldots,j_m)\\ \not\in \{(1,\ldots,1),(2,\ldots,2)\}}}\dfrac{\Pr(\mc{E}_{j_1, \ldots, j_m})\Pr(\mc{E}_{3-j_1,\ldots, 3-j_m})}{2}}\right)
 \end{align*}
 where  $\mc{E}_{j_1, \ldots, j_m}$ denotes the event $\RZ_1^r \in \mc{A}_{1j_1}, \ldots, \RZ_m^r \in \mc{A}_{mj_m}$ for $(j_1,\ldots,j_m) \in \{1, 2\}^m$.
 
%  \item There is an integer $s$, and a non-empty set $\mc{A}_{1}\times\ldots\times\mc{A}_{m}\subset \mc{Z}^s_{1}\times\ldots\times\mc{Z}^s_{m}$ such that 
%  \begin{align}
%      &H(\RZ^s_V|\RZ^s_{\opw},\RZ^s_V\in \mc{A}_{1}\times\ldots\times\mc{A}_{m})
%      \notag \\& \mkern 100mu  > \rco(\RZ^s_V|\RZ^s_V\in \mc{A}_{1}\times\ldots\times\mc{A}_{m})
%  \end{align}

% \item $\rl(\RZ_V||\RZ_{\opw}) < H(\RZ_V|\RZ_{\opw})$.
 \item $\wskc(\RZ_V \| \RZ_{\opw}) > 0$.
 \item $\Delta(\RZ_V \| \RZ_{\opw}) = 0$.
 \item $\Delta(\RZ_V \| \RZ_{\opw}) < \delta_1$ where $\delta_1$ is the smallest root of the equation $16\delta^2-(8+4\sqrt{2^{m-1}-1})\delta+1=0$. (It can be seen that $\delta_1$ is strictly positive for any $m\geq 2$.)
\end{enumerate}
\end{theorem}
% \begin{proof}
%  See Appendix~\ref{app:multivariate_positivity}.
% \end{proof}

{\color{blue}
\begin{IEEEproof}[Proof sketch] Most of the steps in the proof are analogous to the proof for the two-user case \cite[Theorem~4]{amin2020}. We highlight here the fact that we can use our lower bound \eqref{eq:RL:lb} on $\rl$ to prove the statement that 1) implies 2). The idea is to show that if 1) holds then for a transformed source  $(\tRZ_V,\tRZ_{\opw})$ obtained using the sets given in 1),
  \begin{align*} \label{eq:rco_nonmaximal}
     H(\tRZ^n_V \mid \tRZ^n_{\opw},\tRZ^n_V\in \mc{A}_{1}\times\cdots\times\mc{A}_{m})
    %\notag \\& \mkern 100mu  
      -\rco(\tRZ^n_V \mid \tRZ^n_V\in \mc{A}_{1}\times\cdots\times\mc{A}_{m})>0
 \end{align*}
 for some integer $n$, and a positive-probability event $\mc{E}=\big\{\tRZ^n_V\in \mc{A}_{1}\times\cdots\times\mc{A}_{m}\big\}$, where $\mc{A}_{i} \subset \{1,2\}^n$ for all $i \in V$. This step can be argued using the repetition coding with block swapping idea from \cite[Theorem~4]{amin2020}. By using the bound $\rco \geq \rl$ and  the lower bound \eqref{eq:RL:lb} on $\wskc$, we have
 \begin{align*}
    n \, \wskc(\tRZ_V\|\tRZ_{\opw}) & =\wskc(\tRZ^n_V\|\tRZ^n_{\opw})\\ & 
    \utag{a}{\geq} \, \Pr(\mc{E})\, \wskc(\tRZ^n_V\parallel\tRZ^n_{\opw},\tRZ^n_V\in \mc{A}_{1}\times\cdots\times\mc{A}_{m})\\
    &\geq\Pr(\mc{E})\left[H(\tRZ^n_V\mid\tRZ^n_{\opw},\tRZ^n_V\in \mc{A}_{1}\times\cdots\times\mc{A}_{m})
          -\rl(\tRZ^n_V\parallel\tRZ^n_{\opw},\tRZ^n_V\in \mc{A}_{1}\times\cdots\times\mc{A}_{m})\right]\\
          & \geq \Pr(\mc{E}) \left[H(\tRZ^n_V\mid\tRZ^n_{\opw},\tRZ^n_V\in \mc{A}_{1}\times\cdots\times\mc{A}_{m})
    %\notag \\& \mkern 100mu  
      -\rco(\tRZ^n_V \mid\tRZ^n_V\in \mc{A}_{1}\times\cdots\times\mc{A}_{m})\right]\\
      &>0,
 \end{align*}
 where \uref{a} follows from applying \cite[Lemma~3]{maurer93} to the event $\mc{E}$. The source transformation is done in such a way that $\wskc(\tRZ_V\|\tRZ_{\opw})>0$ implies $\wskc(\RZ_V\|\RZ_{\opw}) > 0$, hence condition 2) follows. The remaining steps are analogous to the two-user case, hence omitted.
\end{IEEEproof}

\medskip

We remark here that we presented the above multiuser extension of the two-user result of Gohari, G\"unl\"u and Kramer \cite[Theorem 4]{amin2020} only to illustrate the point that our inequality $H(\RZ_V|\RZ_{\opw}) - \wskc \leq \rl$ could have its uses beyond the equality case. We do not claim that this is the only way to establish the implication 1) $\Longrightarrow$ 2); indeed, other proofs may well be possible which do not use the notion of $\rl$. It would also be of interest to explore the use of Theorem~\ref{thm:multivariate_positivity} in establishing the positivity of $\wskc$ for some class of multiterminal sources $(\RZ_V, \RZ_{\opw})$, as was done in \cite{amin2020} for the case of erasure sources. However, such an exploration would take us well away from the theme of this paper, so we leave it for future work.

One of the ingredients used in the proof of Theorem~\ref{thm:multivariate_positivity} is a result of Maurer, \cite[Lemma~3]{maurer93}, 
that relates $\wskc$ of a source $(\RZ_V,\RZ_{\opw})$ to the source $(\hat{\RZ}_V,\RZ_{\opw})$ whose distribution is obtained by conditioning the distribution of $(\RZ_V,\RZ_{\opw})$ by a certain event. Formally, given some non-empty sets $\mc{A}_1 \subseteq \mc{Z}_1, \ldots, \mc{A}_m \subseteq \mc{Z}_m$, let $\mc{E}$ denote the event that $\RZ_V \in \mc{A}_{1}\times\cdots\times\mc{A}_{m}$ . Define a new source $(\hat{\RZ}_V,\RZ_{\opw})$ taking values in the same alphabets $\mc{Z}_1, \ldots, \mc{Z}_m$ and $\mc{Z}_{\opw}$ with the probability distribution
\begin{align}\label{eq:hatsource}
    P_{\hat{\RZ}_1 \ldots \hat{\RZ}_m \RZ_{\opw}}(z_1, \ldots, z_m, z_{\opw}) := \dfrac{P_{\RZ_1 \ldots \RZ_m, \RZ_{\opw}}(z_1, \ldots, z_m, z_{\opw})}{\Pr(\mc{E})}
\end{align}
if $(z_1, \ldots, z_m) \in \mc{A}_{1}\times\cdots\times\mc{A}_{m}$, and $P_{\hat{\RZ}_1 \ldots \hat{\RZ}_m \RZ_{\opw}}(z_1, \ldots, z_m, z_{\opw}) := 0$ otherwise.
It was shown in \cite[Lemma~3]{maurer93} that  $\wskc(\RZ_V\|\RZ_{\opw})\geq\Pr(\mc{E})\wskc(\hat{\RZ}_V\|\RZ_{\opw})$. The minimum leakage rate for omniscience $\rl$ also satisfies a similar relation.

\begin{lemma}\label{lem:hatsource}
For sources $(\RZ_V,\RZ_{\opw})$ and $(\hat{\RZ}_V,\RZ_{\opw})$, which is defined as above for some event $\mc{E}:=\{\RZ_V \in \mc{A}_{1}\times\cdots\times\mc{A}_{m}\}$, we have 
\begin{align}
    &H(\RZ_V|\RZ_{\opw})-\rl(\RZ_V\|\RZ_{\opw}) %\notag \\& \mkern 100mu 
    \geq \Pr(\mc{E})[H(\hat{\RZ}_V|\RZ_{\opw})-\rl(\hat{\RZ}_V\|\RZ_{\opw})]
\end{align}
\end{lemma}
\begin{proof}
Let $\hat{\RF}^{(n)}$ be an omniscience scheme for the source $\hat{\RZ}_V$ that achieves $\rl(\hat{\RZ}_V\|\RZ_{\opw})$. We will construct an omniscience scheme for the source $\RZ_V$ with the leakage rate $H(\RZ_V|\RZ_{\opw})-\Pr(\mc{E})[H(\hat{\RZ}_V|\RZ_{\opw})-\rl(\hat{\RZ}_V\|\RZ_{\opw})]$, which proves the lemma. Fix a large enough $n$ and consider $n$ i.i.d. realizations of the source  $(\RZ_V,\RZ_{\opw})$. In the first phase of communication, each user reveals publicly the indices of those realizations that fall in their corresponding set $\mcA_i$ to the other users. For instance, user $i$ transmits $\RF_{1,i}(\RZ_i^n):= (b_{ij} : b_{ij} = \mathbf{1}_{\mcA_i}(\RZ_{ij}), 1\leq j\leq n)$, which is a sequence indicating the locations where $\RZ_{ij} \in \mcA_i$. This communication involves $m$ message transmissions. At the end of the first phase, through $(\RF_{1,i}: i \in V)$, every user knows the indices where the event $\mcE$ has occurred, i.e., $\mcE$ occurs at an index $j$ if $b_{ij}=1$ for all $i \in V$.  

In the second phase of communication, users discuss interactively based on the first phase of communication. Let $\mcJ$ denote the set of indices for which $\mcE$ occurs. On the indices in $\mcJ^c$, users reveal their complete observations. For example, user $i$ communicates $\RF_{2,i}(\RZ_i^n, \RF_{1,1}, \ldots, \RF_{1,m}):= \RZ_{i,\mcJ^c}$. And, for the block corresponding to $\mcJ$, they communicate according to $\hat{\RF}^{(\mcJ)}$, which is in general interactive. And, the corresponding communication is $\RF_3:=\hat{\RF}^{(\mcJ)}(\RZ^n_V)$, which acts only on the block corresponding to $\mcJ$. Note that conditioning on a realization $\mcJ=J \subset [n]$, the distribution of  $(\RZ_{V,J},\RZ_{\opw,J})$ is the same as that of $|J|$ i.i.d. realizations of $(\hat{\RZ}_V,\RZ_{\opw})$. 

Let $(\RC_j:1\leq j\leq n)$ be a random sequence where $\RC_j = \mathbf{1}_{\mc{A}_{1}\times\cdots\times\mc{A}_{m}}(\RZ_{V,j})$, and observe that this is an i.i.d. sequence. Using the strong typicality of this sequence, it is easy to verify that the communication $\RF^{(n)}:= (\RF_{1,1}, \ldots, \RF_{1,m},\RF_{2,1}, \ldots, \RF_{2,m},\RF_3)$ satisfies the recoverability condition \eqref{eq:omn:recoverability} for omniscience.  The leakage rate is 
\begin{align*}
    \frac{1}{n} I(\RZ_V^{n} \wedge \RF^{(n)} \mid \RZ_{\opw}^n) = H(\RZ_V \mid \RZ_{\opw}) - \frac{1}{n}H(\RZ_V^{n} \mid \RF^{(n)}, \RZ_{\opw}^n).
\end{align*}

Consider the term $\frac{1}{n}H(\RZ_V^{n} \mid \RF^{(n)}, \RZ_{\opw}^n)$ which, from the form of the communication $\RF^{(n)}$, can be seen to be equal to $\frac{1}{n}H(\RZ_{V,\mcJ} \mid \mcJ, \hat{\RF}^{(\mcJ)}, \RZ_{\opw,\mcJ})$, which we write as $\frac{1}{n}[H(\RZ_{V,\mcJ} \mid \mcJ, \RZ_{\opw,\mcJ})-I(\RZ_{V,\mcJ} \wedge  \hat{\RF}^{(\mcJ)}\mid \mcJ, \RZ_{\opw,\mcJ})]$. The first of these terms can be readily single-letterized:
\begin{align*}
    \frac{1}{n}H(\RZ_{V,\mcJ} \mid \mcJ, \RZ_{\opw,\mcJ}) &= \frac{1}{n}\sum_{J \subseteq [n]} \Pr(\mcJ = J) H(\RZ_{V,J} | \mcJ = J, \RZ_{\opw,J}) \\
    &= \frac{1}{n}\sum_{J \subseteq [n]} \Pr(\mcJ = J) \, |J| \, H(\hat{\RZ}_V|\RZ_{\opw}) \\
    &= \mathbb{E}\left[\frac{|\mcJ|}{n}\right] \, H(\hat{\RZ}_V|\RZ_{\opw})  \ = \ \Pr(\mc{E}) \, H(\hat{\RZ}_V|\RZ_{\opw}).
\end{align*}
It can be easily shown that $\liminf_{n\to \infty}\frac{1}{n}H(\RZ_{V,\mcJ} \mid \mcJ, \hat{\RF}^{(\mcJ)}, \RZ_{\opw,\mcJ})  \geq  \Pr(\mc{E})[H(\hat{\RZ}_V|\RZ_{\opw})-\rl(\hat{\RZ}_V|\RZ_{\opw})]$ for an $\rl(\hat{\RZ}_V\|\RZ_{\opw})$-optimal omniscience scheme  $\hat{\RF}^{(n)}$.
Thus we have 
\begin{align*}
    \rl(\RZ_V\|\RZ_{\opw}) &\leq \limsup_{n \to \infty} \frac{1}{n} I(\RZ_V^{n} \wedge \RF^{(n)} \mid \RZ_{\opw}^n) \\ & \leq H(\RZ_V|\RZ_{\opw})%\\& \mkern 50mu
    -\Pr(\mc{E})[H(\hat{\RZ}_V|\RZ_{\opw})-\rl(\hat{\RZ}_V\|\RZ_{\opw})].
\end{align*}
This completes the proof.
\end{proof} 
}








==> proof_lessnoisy.tex <==
 First let us show that $\RZ$ is more capable than $\RY$ iff $\epsilon \leq h(p)$. Let $P_{\RX}=(P_{\RX}(0), P_{\RX}(1)):=(q, 1-q)$, and $I(\RX\wedge\RZ) - I(\RX\wedge\RY) = (1-\epsilon)h(q) - h(p*q) +h(p) \triangleq f(q)$ where $q \in [0,1]$ and $p*q=p(1-q)+(1-p)q$. If $\epsilon > h(p)$, then $f(\frac{1}{2})= h(p) - \epsilon < 0$ which implies that $\RZ$ is not more capable than $\RY$. For the other direction, we can use the convexity \cite[Lemma~2]{wynergerber} of the function $h(p*h^{-1}(x))$, $0\leq x \leq 1$. For $x_1=0$, $x_2=1$ and $\lambda= 1- h(q)$, we have $(1-h(q))h(p)+h(q)=\lambda h(p*h^{-1}(x_1))+(1-\lambda)h(p*h^{-1}(x_2))\geq h(p*h^{-1}(\lambda x_1 +(1-\lambda)x_2)) =  h(p*h^{-1}(h(q)))=h(p*\min\{q, 1-q\})= h(p*q)$.  Hence if $\epsilon \leq h(p)$ then $f(q) \geq (1-h(p))h(q) - h(p*q) +h(p) \geq 0$, where the last inequality uses the convexity result. This proves that $\RZ$ is more capable than $\RY$.
 
 Next we will show that $\RZ$ is less noisy than $\RY$ iff $\epsilon \leq 4p(1-p)$. Proving that $\RZ$ is less noisy than $\RY$ is equivalent to proving the concavity of  $I(\RX\wedge\RZ) - I(\RX\wedge\RY)$ with respect to the input distribution $P_{\RX}$ \cite[p.~126]{elgamalbook}. This follows from the observation that for $\RU-\RX-(\RY, \RZ)$,   $I(\RU\wedge\RZ) - I(\RU\wedge\RY) = I(\RX\wedge\RZ) - I(\RX\wedge\RY) - \big[I(\RX\wedge\RZ|\RU) - I(\RX\wedge\RY| \RU)\big]$. So it is enough to prove that $f(q), 0 \leq q \leq 1,$ is concave iff $\epsilon \leq 4p(1-p)$. The first and second derivatives are $f'(q)=(1-\epsilon)h'(q) - (1-2p)h'(p*q)$ and $f''(q)=(1-\epsilon)h''(q) - (1-2p)^2h''(p*q)$ for $0 \leq q \leq 1$. If $\epsilon \leq 4p(1-p)$ then $(1-\epsilon) \geq (1-2p)^2$ and $f''(q)\leq (1-\epsilon)[h''(q) - h''(p*q)]$. The function $h''(x)= \frac{1}{\ln 2}\left(\frac{-1}{x(1-x)}\right)$ is strictly increasing in the interval $(0,\frac{1}{2}]$, and is strictly decreasing in the interval $[\frac{1}{2}, 1)$. Since $p \in(0, \frac{1}{2})$, $q < p*q < \frac{1}{2}$ if $q < \frac{1}{2}$, $  \frac{1}{2}< p*q < q$ if $q > \frac{1}{2}$, and $p*q = q$  if $q=\frac{1}{2}$. In all these cases, $h''(q) - h''(p*q)\leq 0$ which implies that $f(q)$ is concave.  If $\epsilon > 4p(1-p)$ then $f''(\frac{1}{2})= \frac{1}{\ln 2}[-(1-\epsilon)+(1-2p)^2] >0 $, and hence $f(q)$ is not concave. 
 Since $f'(\frac{1}{2}) = 0$ and $f''(\frac{1}{2})>0$, $f(q)$, which is a symmetric function around $q=\frac{1}{2}$, is also strictly convex in a neighbourhood of $q=\frac{1}{2}$. Therefore, we have $f(\frac{1}{2})< \frac{1}{2}f(\frac{1}{2}+\delta)+\frac{1}{2}f(\frac{1}{2}-\delta)$ for some $\delta>0$. Let $\RU$ be a binary random variable with distribution Ber$(\frac{1}{2})$ and $\RX$ is obtained by passing $\RU$ through BSC$(\frac{1}{2}-\delta)$. For this choice of $P^*_{\RU,\RX}$, $I(\RU\wedge\RZ) - I(\RU\wedge\RY)=I(\RX\wedge\RZ) - I(\RX\wedge\RY) - \big[I(\RX\wedge\RZ|\RU) - I(\RX\wedge\RY| \RU)\big] = f(\frac{1}{2})- \big[\frac{1}{2}f(\frac{1}{2}+\delta)+\frac{1}{2}f(\frac{1}{2}-\delta)\big]< 0$. 



==> proof_multivariate_positivity.tex <==
Some of the steps in the proof are analogous to the proof for the two-user case, \cite[Theorem~4]{amin2020}.  The new component of the theorem is the identification of a connection between the positivity of $\wskc$ and the non-maximality of $\rl$ of a transformed source.
Since most of the essential ideas of the two-user setting work even in the multiuser case, we only give proof sketches for these analogous steps. However, the new arguments are described in detail.


% we only provide new key arguments  and give proof sketches for the analogous arguments.

The statement 3) implies 4) is trivial. So it is enough to show that 1) implies 2), 2) implies 3), and 4) implies 1).

\textit{1) implies 2):} We prove this by following an approach that is similar to that of the two-user case. First, using the sets given in 1), we construct a new source $(\tRZ_V,\tRZ_{\opw})$ by applying some functions to the user random variables of the source $(\RZ^r_V,\RZ^r_{\opw})$. Then, we show that $\wskc(\tRZ_V||\tRZ_{\opw})>0$ which in turn implies that $\wskc(\RZ_V||\RZ_{\opw})>0$ because any SKA scheme on the source $(\tRZ_V,\tRZ_{\opw})$ is an SKA scheme on $(\RZ_V,\RZ_{\opw})$. To prove $\wskc(\tRZ_V||\tRZ_{\opw})>0$ using condition 1), we use the lower bound of Theorem~\ref{thm:RL:lb} and Lemma~\ref{lem:hatsource} for the new source.


Let $(\tRZ_1,\ldots,\tRZ_m,\tRZ_{\opw})$ be a function of $(\RZ^r_1,\ldots,\RZ^r_m,\RZ^r_{\opw})$ obtained by setting $\tRZ_i = 1$ if $\RZ_i^r \in \mc{A}_{i1}$, $\tRZ_i = 2$ if $\RZ_i^r \in \mc{A}_{i2}$ and  $\tRZ_i = 3$ if $\RZ_i^r \not\in \mc{A}_{i1}\cup \mc{A}_{i2}$ for $1\leq i\leq m$, and $\tRZ_{\opw} = \RZ_{\opw}^r$. Let $p_{j_1\ldots j_m} :=\Pr(\tRZ_1=j_1, \ldots, \tRZ_m=j_m)= \Pr(\RZ^r_1 \in \mcA_{1j_1}, \ldots, \tRZ_m\in \mcA_{mj_m})$ for all $(j_1, \ldots, j_m) \in \{1,2\}^m$. The condition in 1) is equivalent  to the condition 
\begin{align*}
       &D_{\frac{1}{2}} \left(P_{\tRZ_{\opw}}(.|\tRZ_1=1, \ldots, \tRZ_m=1)  
       %\right. \\& \mkern 100mu \left.
       ||P_{\tRZ_{\opw}}(.|\tRZ_1=2, \ldots, \tRZ_m=2) \right)
       < \log \left(\frac{p_{1,1,\ldots,1}p_{2,2,\ldots,2}}{\sum \limits_{\substack{(j_1,\ldots,j_m)\\ \not\in \{(1,\ldots,1),\\\mkern 30mu (2,\ldots,2)\}}}\dfrac{p_{j_1, \ldots, j_m}p_{3-j_1,\ldots, 3-j_m}}{2}}\right).
 \end{align*}
 
 
 We will show that the above condition implies 
  \begin{align} \label{eq:rco_nonmaximal}
     &H(\tRZ^n_V|\tRZ^n_{\opw},\tRZ^n_V\in \mc{A}_{1}\times\cdots\times\mc{A}_{m})
    %\notag \\& \mkern 100mu  
     > \rco(\tRZ^n_V|\tRZ^n_V\in \mc{A}_{1}\times\cdots\times\mc{A}_{m})
 \end{align}
 for some integer $n$, and a non-empty set $\mc{A}_{1}\times\cdots\times\mc{A}_{m}$, where $\mc{A}_{i} \subset \{1,2\}^n$ for all $i \in V$. Because of the following argument, inequality \eqref{eq:rco_nonmaximal} implies that $\wskc(\tRZ_V||\tRZ_{\opw})>0$ which further implies that $\wskc(\RZ_V||\RZ_{\opw})>0$. Suppose that there is an integer $n$, and a non-empty set $\mc{A}_{1}\times\cdots\times\mc{A}_{m}\subset \{1,2\}^n\times\cdots\times \{1,2\}^n$ such that \eqref{eq:rco_nonmaximal} holds. Let $(\widehat{\tRZ_V^n},\tRZ^n_{\opw})$ be the source as defined in \eqref{eq:hatsource} using the source $(\tRZ_V^n,\tRZ^n_{\opw})$ and the set $\mc{A}_{1}\times\cdots\times\mc{A}_{m}$.  Condition \eqref{eq:rco_nonmaximal} can be written as $H(\widehat{\tRZ_V^n}|\tRZ^n_{\opw})> \rco(\widehat{\tRZ_V^n})$. For the new source, it follows from \eqref{eq:rl_rco} that 
 \begin{align*}
     \rl(\widehat{\tRZ_V^n}||\tRZ^n_{\opw}) \leq \rco(\widehat{\tRZ_V^n}).
 \end{align*}
Therefore, we have  $H(\widehat{\tRZ_V^n}|\tRZ^n_{\opw})-\rl(\widehat{\tRZ_V^n}||\tRZ^n_{\opw}) \geq H(\widehat{\tRZ_V^n}|\tRZ^n_{\opw})- \rco(\widehat{\tRZ_V^n})>0$. By combining this with Lemma~\ref{lem:hatsource}, we get 
$H(\tRZ_V^n|\tRZ^n_{\opw})-\rl(\tRZ_V^n||\tRZ^n_{\opw}) \geq \Pr(\mcE) [H(\widehat{\tRZ_V^n}|\tRZ^n_{\opw})-\rl(\widehat{\tRZ_V^n}||\tRZ^n_{\opw})]>0$. So we conclude that $H(\tRZ_V|\tRZ_{\opw})-\rl(\RZ_V||\tRZ_{\opw})=\dfrac{1}{n}[H(\tRZ_V^n|\tRZ^n_{\opw})-\rl(\tRZ_V^n||\tRZ^n_{\opw})]>0$. Hence, it follows from the lower bound of Theorem~\ref{thm:RL:lb} that if $\rl(\tRZ_V||\tRZ_{\opw})< H(\tRZ_V|\tRZ_{\opw})$ then $\wskc(\tRZ_V||\tRZ_{\opw})>0$. Since the source $(\tRZ_V, \tRZ_{\opw})$ is obtained by processing (deterministically) each user observations of the source $(\RZ^r_V, \RZ^r_{\opw})$, any positive rate secret key on $(\tRZ_V, \tRZ_{\opw})$ is also a positive rate secret key on $(\RZ^r_V, \RZ^r_{\opw})$. Thus $\wskc(\tRZ_V||\tRZ_{\opw})>0$ implies that $\wskc(\RZ_V||\RZ_{\opw})= \frac{1}{r}\wskc(\RZ^r_V|| \RZ^r_{\opw})>0$.\\


Now we will show  that condition 1) implies \eqref{eq:rco_nonmaximal}.
Consider the following repetition coding with block swapping: for an even integer $n$, let
 \begin{align*}
  \mathbf{1}&:=\underbrace{1\ldots 1}_{n/2}\underbrace{ 2\ldots 2}_{n/2}\\
  \mathbf{2}&:=2\ldots 2 1\ldots 1
 \end{align*}
 and $\mc{A}_{i}:=\{\mathbf{1},\mathbf{2}\}$, for $1\leq i\leq m$. Let us define $\mc{A}_{V}:=\mc{A}_{1}\times\cdots\times\mc{A}_{m}$. It is enough to show that for large enough $n$, 
\begin{align}\label{eq:non_maximal_1}
     H(\tRZ^n_V|\tRZ^n_{\opw},\tRZ^n_V\in \mc{A}_{V}) > \rco(\tRZ^n_V|\tRZ^n_V\in \mc{A}_{V}).
 \end{align}
 Let $\mc{B}:=2^V \backslash \{\emptyset, V\}$, $\lambda^{(n)}$ be a fractional partition of $\mc{B}$, i.e., $\lambda^{(n)}:\mc{B} \to \mathbb{R}^+$ is such that $\sum_{i\in B}\lambda^{(n)}(B)=1$ for every $i \in V$; and let $\Lambda^{(n)}$ be the set of all fractional partitions. The minimum rate of communication for omniscience \cite[Sec. V]{csiszar04} is given by
 \begin{align*} 
     &\rco(\tRZ^n_V|\tRZ^n_V\in \mc{A}_{V})%\\ & \mkern 70mu
     = \max \limits_{\lambda^{(n)} \in \Lambda^{(n)}} \sum \limits_{B \in \mc{B}} \lambda^{(n)}_B H(\tRZ^n_B|\tRZ^n_{B^c},\tRZ^n_V\in \mc{A}_{V}).
 \end{align*}
Though the optimal fractional partition seems to depend on $n$, because of the repetitive structure of the coding this dependence disappears. We can upper bound $\rco$ as 
 \begin{align}\label{eq:non_maximal_2}
  \rco(\tRZ^n_V|\tRZ^n_V\in \mc{A}_{V})\notag%\\&\mkern 70mu
  &= \max \limits_{\lambda^{(n)} \in \Lambda^{(n)}} \sum \limits_{B \in \mc{B}} \lambda^{(n)}_B H(\tRZ^n_B|\tRZ^n_{B^c},\tRZ^n_V\in \mc{A}_{V})\notag\\
  &= \sum \limits_{B \in \mc{B}} \lambda^{*(n)}_B H(\tRZ^n_B|\tRZ^n_{B^c},\tRZ^n_V\in \mc{A}_{V})\notag\\
  &\leq \sum \limits_{B \in \mc{B}}H(\tRZ^n_B|\tRZ^n_{B^c},\tRZ^n_V\in \mc{A}_{V})\notag\\
  &\leq (2^{m}-2)\max \limits_{i \in V} H(\tRZ^n_{V \backslash i}|\tRZ^n_{i},\tRZ^n_V\in \mc{A}_{V}),
 \end{align}
 where we used in the first inequality that the optimal fractional partition $\lambda^{*(n)}_B$ is bounded above by $1$ for all $B \in \mc{B}$, and in the last inequality that  $H(\tRZ^n_B|\tRZ^n_{B^c},\tRZ^n_V\in \mc{A}_{V}) \leq \max \limits_{i \in V} H(\tRZ^n_{V \backslash i}|\tRZ^n_{i},\tRZ^n_V\in \mc{A}_{V})$ for all $B \in \mc{B}$.\\
 
 
% Since $\rco(\tRZ^n_V|\tRZ^n_V\in \mc{A}_{V})$ is upper bounded by $(2^{m}-2)\max \limits_{i \in V} H(\tRZ^n_{V \backslash i}|\tRZ^n_{i},\tRZ^n_V\in \mc{A}_{V})$,  it suffices to prove \begin{align*}
%     &H(\tRZ^n_V|\tRZ^n_{\opw},\tRZ^n_V\in \mc{A}_{V})
%     \\& \mkern 70mu > (2^{m}-2)\max \limits_{i \in V} H(\tRZ^n_{V \backslash i}|\tRZ^n_{i},\tRZ^n_V\in \mc{A}_{V}).
% \end{align*}
Let us further upper bound $(2^{m}-2)\max \limits_{i \in V} H(\tRZ^n_{V \backslash i}|\tRZ^n_{i},\tRZ^n_V\in \mc{A}_{V})$ as follows. Consider the term $H(\tRZ^n_{V \backslash i_0}|\tRZ^n_{i_0},\tRZ^n_V\in \mc{A}_{V})$ for some $i_0 \in V$. We know that 
 \begin{align*}
  \Pr[\tRZ^n_1= \mathbf{k}_1,\ldots,\tRZ^n_m=\mathbf{k}_m]= p_{k_1\ldots k_m}^{n/2}p_{3-k_1\ldots 3-k_m}^{n/2}
 \end{align*}
for all $(\mathbf{k}_1, \ldots, \mathbf{k}_m) \in \{\mathbf{1},\mathbf{2}\}^m$, and for $i \in V$, $k_i$ denotes the first symbol in the sequence $\mathbf{k}_i$. Therefore, we get
\begin{align*}
  \Pr[\tRZ^n_1=\mathbf{k}_1,\ldots,\tRZ^n_m=\mathbf{k}_m|\tRZ^n_V\in \mc{A}_{V}]%\\&\mkern 70mu
  = \dfrac{p_{k_1\ldots k_m}^{n/2}p_{3-k_1\ldots 3-k_m}^{n/2}}{\sum \limits_{\substack{(j_1,\ldots,j_m)\in \{1,2\}^m}}p_{j_1\ldots j_m}^{n/2}p_{3-j_1\ldots 3-j_m}^{n/2}}.
 \end{align*}
For $i_0 \in V$ and $(\mathbf{k}_1, \ldots, \mathbf{k}_m) \in \{\mathbf{1},\mathbf{2}\}^m$, we have 
 \begin{align*}
  \Pr[\tRZ^n_{V \backslash i_0}=\mathbf{k}_{V \backslash i_0} |\tRZ^n_{i_0}=\mathbf{k}_{i_0}, \tRZ^n_V\in \mc{A}_{V}]
  %& = \dfrac{p_{k_1\ldots k_{i_0}\ldots k_m}^{n/2}p_{3-k_1\ldots 3-k_{j_0}\ldots 3-k_m}^{n/2}}{\sum \limits_{\substack{(j_1,\ldots,k_{i_0},\ldots,j_m)\in \{1,2\}^m}}p_{j_1\ldots k_{i_0}\ldots j_m}^{n/2}p_{3-j_1\ldots 3-k_{i_0}\ldots 3-j_m}^{n/2}}\\
  %\\&\mkern 70mu 
  = \dfrac{p_{k_1\ldots k_{i_0}\ldots k_m}^{n/2}p_{3-k_1\ldots 3-k_{j_0}\ldots 3-k_m}^{n/2}}{\dfrac{1}{2}\sum \limits_{\substack{(j_1,\ldots,j_m)\in \{1,2\}^m}}p_{j_1\ldots j_m}^{n/2}p_{3-j_1\ldots 3-j_m}^{n/2}}
 \end{align*}
 where the equality follows from the symmetry in the probabilities of the sequences $(j_1,\ldots,k_{i_0},\ldots,j_m)$ and $(3-j_1,\ldots,3-k_{i_0},\ldots,3-j_m)$. To compute the entropies, we make use of the grouping property of the entropy: For a probability vector $(q_1, q_2, \ldots, q_s)$, $H(q_1, q_2,.....,q_s)= H\left(q_1, q_2+ \cdots+q_s\right)+ (q_2+ \cdots+q_s)H \Big(\dfrac{q_2}{q_2+ \cdots+q_s},\ldots,\linebreak \dfrac{q_s}{q_2+ \cdots+q_s}\Big)$. If $q_1 \in [0.5, 1]$, then $h(q_1)\leq - 2(1-q_1)\log_2 (1-q_1)$ which implies $H(q_1, q_2,.....,q_s)\leq h(q_1)+(1-q_1)\log_2 (s-1) \leq (1-q_1)\log_2 (s-1) - 2(1-q_1)\log_2 (1-q_1)$. Note that because R\'enyi divergence is non-negative, the inequality in 1) implies that
\begin{align*}
    p_{1\ldots 1}p_{2\ldots 2}& >  \dfrac{1}{2}\sum \limits_{\substack{(j_1,\ldots,j_m)\\ \not\in \{(1,\ldots,1),(2,\ldots,2)\}}}p_{j_1, \ldots, j_m}p_{3-j_1,\ldots, 3-j_m}. %\\ & \geq \dfrac{1}{2}p_{j_1, \ldots, j_m}p_{3-j_1,\ldots, 3-j_m}.
\end{align*}
So, by setting 
 \begin{align*}
     q^{(n)}_1 &:= \dfrac{p_{1\ldots 1}^{n/2}p_{2\ldots 2}^{n/2}}{\dfrac{1}{2}\sum \limits_{\substack{(j_1,\ldots,j_m)\in \{1,2\}^m}}p_{j_1\ldots j_m}^{n/2}p_{3-j_1\ldots 3-j_m}^{n/2}}= \dfrac{p_{1\ldots 1}^{n/2}p_{2\ldots 2}^{n/2}}{p_{1\ldots 1}^{n/2}p_{2\ldots 2}^{n/2}+\dfrac{1}{2}\sum \limits_{\substack{(j_1,\ldots,j_m)\\ \not\in \{(1,\ldots,1),(2,\ldots,2)\}}}p_{j_1\ldots j_m}^{n/2}p_{3-j_1\ldots 3-j_m}^{n/2}},
 \end{align*} 
 which is greater than $1/2$, we have for any $i_0 \in V$, 
 \begin{align}\label{eq:non_maximal_3}
    &H(\tRZ^n_{V \backslash i_0}|\tRZ^n_{i_0},\tRZ^n_V\in \mc{A}_{V})%\notag \\& \mkern 30mu 
    \leq (1-q^{(n)}_1)(\log_2 (2^{m-1}-1) - 2\log_2 (1-q^{(n)}_1)).
\end{align}
where we replaced $s$ by $2^{m-1}$. Notice that the bound is independent of $i_0$. Therefore, from \eqref{eq:non_maximal_2} and \eqref{eq:non_maximal_3}, we have 
\begin{align*}
 &\rco(\tRZ^n_V|\tRZ^n_V\in \mc{A}_{V})%\\& 
 \leq (2^{m}-2)[(1-q^{(n)}_1)(\log_2 (2^{m-1}-1) - 2\log_2 (1-q^{(n)}_1))].\notag
\end{align*}
Because of the above inequality, it is enough prove that condition 1) implies 
\begin{align}\label{eq:final}
 &H(\tRZ^n_V|\tRZ^n_{\opw},\tRZ^n_V\in \mc{A}_{V})%\\& 
 > (2^{m}-2)[(1-q^{(n)}_1)(\log_2 (2^{m-1}-1) - 2\log_2 (1-q^{(n)}_1))].%\notag
\end{align}

Now let us argue that condition 1) implies \eqref{eq:final}. Since 
\begin{align*}
 q^{(n)}_1&= \dfrac{p_{1\ldots 1}^{n/2}p_{2\ldots 2}^{n/2}}{p_{1\ldots 1}^{n/2}p_{2\ldots 2}^{n/2}+\dfrac{1}{2}\sum \limits_{\substack{(k_1,\ldots,k_m) \not\in\\  \{(1,\ldots,1),(2,\ldots,2)\}}}p_{k_1\ldots k_m}^{n/2}p_{3-k_1\ldots 3-k_m}^{n/2}}\\ &\geq \dfrac{p_{1\ldots 1}^{n/2}p_{2\ldots 2}^{n/2}}{p_{1\ldots 1}^{n/2}p_{2\ldots 2}^{n/2}+\left(\dfrac{1}{2} \sum \limits_{\substack{(k_1,\ldots,k_m)\not\in \\  \{(1,\ldots,1),(2,\ldots,2)\}}}p_{k_1\ldots k_m}p_{3-k_1\ldots 3-k_m}\right)^{\frac{n}{2}}},
\end{align*}
 we have
$$\lim \limits_{n \to \infty}(1-q^{(n)}_1)^{\frac{1}{n}} \leq \sqrt{\dfrac{\dfrac{1}{2} \sum \limits_{\substack{(k_1,\ldots,k_m)\\ \not\in \{(1,\ldots,1),(2,\ldots,2)\}}}p_{k_1\ldots k_m}p_{3-k_1\ldots 3-k_m}}{p_{1\ldots 1}p_{2\ldots 2}}} $$
and 
% \begin{align}\label{eq:left_limit}
%     &\lim \limits_{n \to \infty} (2^{m}-2)^{1/n}[(1-q^{(n)}_1)(\log_2 (2^{m-1}-1)  \nonumber \\ & \mkern 150mu - 2\log_2 (1-q^{(n)}_1))]^{1/n} \nonumber \\&\leq \sqrt{\dfrac{\dfrac{1}{2} \sum \limits_{\substack{(k_1,\ldots,k_m)  \\ \not\in \{(1,\ldots,1),(2,\ldots,2)\}}}p_{k_1\ldots k_m}p_{3-k_1\ldots 3-k_m}}{p_{1\ldots 1}p_{2\ldots 2}}}.
% \end{align}
\begin{align}\label{eq:left_limit}
   & \lim \limits_{n \to \infty} (2^{m}-2)^{1/n}[(1-q^{(n)}_1)(\log_2 (2^{m-1}-1) - 2\log_2 (1-q^{(n)}_1))]^{1/n} \nonumber \\ &\mkern 300mu\leq \sqrt{\dfrac{\dfrac{1}{2} \sum \limits_{\substack{(k_1,\ldots,k_m)  \\ \not\in \{(1,\ldots,1),(2,\ldots,2)\}}}p_{k_1\ldots k_m}p_{3-k_1\ldots 3-k_m}}{p_{1\ldots 1}p_{2\ldots 2}}}.
\end{align}
For the asymptotics of the conditional entropy term, we can use the same idea of hypothesis testing at the wiretapper side with $u_1=(\mathbf{1}, \ldots, \mathbf{1})$ and $u_2=(\mathbf{2}, \ldots, \mathbf{2})$ used in \cite[Lemma~2]{amin2020} to get
%  \begin{align}\label{eq:right_limit}
%  &\liminf_{n \to \infty} H(\tRZ^n_V|\tRZ^n_{\opw},\tRZ^n_V\in \mc{A}_{V})^{\frac{1}{n}} \nonumber\\ &\geq  \exp \Big(-\frac{1}{2}D_{\frac{1}{2}} \big(P_{\tRZ_{\opw}}(.|\tRZ_1=1, \ldots, \tRZ_m=1)\nonumber \\& \mkern 150mu  ||P_{\tRZ_{\opw}}(.|\tRZ_1=2, \ldots, \tRZ_m=2) \big)\Big).
%  \end{align}
 \begin{align}\label{eq:right_limit}
 &\liminf_{n \to \infty} H(\tRZ^n_V|\tRZ^n_{\opw},\tRZ^n_V\in \mc{A}_{V})^{\frac{1}{n}} \geq  \exp \Big(-\frac{1}{2}D_{\frac{1}{2}} \big(P_{\tRZ_{\opw}}(.|\tRZ_1=1, \ldots, \tRZ_m=1)  ||P_{\tRZ_{\opw}}(.|\tRZ_1=2, \ldots, \tRZ_m=2) \big)\Big).
 \end{align}


 

Since 
\begin{align*}
       &D_{\frac{1}{2}} \left(P_{\tRZ_{\opw}}(.|\tRZ_1=1, \ldots, \tRZ_m=1)  
       %\right. \\& \mkern 100mu \left.
       ||P_{\tRZ_{\opw}}(.|\tRZ_1=2, \ldots, \tRZ_m=2) \right)
       < \log \left(\frac{p_{1,1,\ldots,1}p_{2,2,\ldots,2}}{\sum \limits_{\substack{(j_1,\ldots,j_m)\\ \not\in \{(1,\ldots,1),\\\mkern 30mu (2,\ldots,2)\}}}\dfrac{p_{j_1, \ldots, j_m}p_{3-j_1,\ldots, 3-j_m}}{2}}\right),
 \end{align*}
 we can conclude from \eqref{eq:left_limit} and \eqref{eq:right_limit} that 
for large enough $n$, \eqref{eq:final} holds. This completes the proof of 1) implies 2).
 
\textit{2) implies 3):} Since the proof follows the same argument as in two user case, we omit most of the details and give only those steps that involve different constants. Following are the multivariate analogues of \cite[eq.~(118) and eq.~(124)]{amin2020}: 
\begin{align*}
    I(\RK_1,\ldots,\RK_m \wedge \RZ^n_{\opw}, \RF^{(n)}) \leq (m+1)\delta+h(\delta)
\end{align*}
and 
\begin{align*}
    &||P_{\RK_1,\ldots, \RK_m,\RF^{(n)},\RZ^n_{\opw}}-P_{\RK_1,\ldots, \RK_m}.P_{\RF^{(n)},\RZ^n_{\opw}}||_{TV}  \leq \sqrt{\frac{(m+1)\delta + h(\delta)}{2}}.
\end{align*}
Using the above inequalities, we get 
\begin{align*}
    &||P_{\RK_1,\ldots, \RK_m,\RF^{(n)},\RZ^n_{\opw}}-\dfrac{1}{2}\mathbf{1}_{\RK_1=\ldots=\RK_m}.P_{\RF^{(n)},\RZ^n_{\opw}}||_{TV}  \leq
    \sqrt{\frac{(m+1)\delta + h(\delta)}{2}}+2\delta
\end{align*}
As $\delta$ can be made arbitrarily close to 0, the condition 3) follows.

\textit{4) implies 1):} To prove this, we need the multivariate analogue of \cite[Lemma~3]{amin2020}. It says that for some sets  $\mc{A}_{11},\mc{A}_{12} \subset \mc{Z}_1^r$, $\mc{A}_{21},\mc{A}_{22} \subset \mc{Z}_2^r$, $\ldots, \mc{A}_{m1},\mc{A}_{m2} \subset \mc{Z}_m^r$,

\begin{align*}
       &\frac{1}{2}D_{\frac{1}{2}} \left(P_{\RZ_{\opw}^r}(.|\mc{E}_{1, 1, \ldots, 1})  
       %\right. \\& \mkern 100mu \left.
       ||P_{\RZ_{\opw}^r}(.|\mc{E}_{2, 2, \ldots, 2}) \right) \leq -\log(1-4\delta),
 \end{align*}
 
\begin{align*} 
& \frac{1}{2}\log \left(\frac{\Pr(\mc{E}_{1, \ldots, 1})\Pr(\mc{E}_{2, \ldots, 2})}{\sum \limits_{\substack{(j_1,\ldots,j_m)\\ \not\in \{(1,\ldots,1),(2,\ldots,2)\}}}\dfrac{\Pr(\mc{E}_{j_1, \ldots, j_m})\Pr(\mc{E}_{3-j_1,\ldots, 3-j_m})}{2}}\right)>\log\left(\dfrac{(\frac{1}{2}-2\delta)}{2\delta\sqrt{2^{m-1}-1}}\right)
 \end{align*}
 where  $\mc{E}_{j_1, \ldots, j_m}$ denotes the event $\RZ_1^r \in \mc{A}_{1j_1}, \ldots, \RZ_m^r \in \mc{A}_{mj_m}$ for $(j_1,\ldots,j_m) \in \{1, 2\}^m$ and $\delta:=||P_{\RK_1,\ldots, \RK_m,\RF^{(r)},\RZ^r_{\opw}}-\dfrac{1}{2}\mathbf{1}_{\RK_1=\dots=\RK_m}.P_{\RF^{(r)},\RZ^r_{\opw}}||_{TV}$. The proof is similar to the two-user case with the following sets $\mc{A}_{ij}=\{z^r_i:\RK_i(z^r_i,f)=j\}$ for all $1\leq i\leq m$ and $j\in\{1,2\}$ where $F^{(r)}=f$ is a realization of the public discussion such that $\delta>||P_{\RK_1,\ldots, \RK_m,\RZ^r_{\opw}|\RF^{(r)}=f}-\dfrac{1}{2}\mathbf{1}_{\RK_1=\ldots=\RK_m}.P_{\RZ^r_{\opw}|\RF^{(r)}=f}||_{TV}$.
 
 Since the condition in 4) implies that any $\delta \leq \delta_1$ satisfies 
\begin{align*}
    -\log(1-4\delta) < \log\left(\dfrac{(\frac{1}{2}-2\delta)}{2\delta\sqrt{2^{m-1}-1}}\right),
\end{align*}
the condition 1) follows. 


